Measuring Approximate Functional Dependencies: a Comparative Study

Approximate functional dependencies (AFDs) are functional dependencies (FDs) that "almost" hold in a relation. While various measures have been proposed to quantify the level to which an FD holds approximately, they are difficult to compare and it is unclear which measure is preferable when one needs to discover FDs in real-world data, i.e., data that only approximately satisfies the FD. In response, this paper formally and qualitatively compares AFD measures. We obtain a formal comparison through a novel presentation of measures in terms of Shannon and logical entropy. Qualitatively, we perform a sensitivity analysis w.r.t. structural properties of input relations and quantitatively study the effectiveness of AFD measures for ranking AFDs on real world data. Based on this analysis, we give clear recommendations for the AFD measures to use in practice.

==> sections/benchmarks.tex <==
\input{sections/rwd-benchmark}
\input{sections/syn-benchmark}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main/main"
%%% End:


==> sections/evaluation.tex <==
We compare the effectiveness of the described \afd measures on three benchmarks:
(i) \rwd: a %collection 
set of real-world tables for which we have manually created
the design schema that serves as the ground truth for comparison; (ii) \nrwd:
obtained from \rwd by adding errors in a controlled fashion to
design \fds that are fully satisfied in \rwd; and, (iii) \syn: a synthetically
generated benchmark. These benchmarks  are discussed in detail together with their evaluation goals in
Section~\ref{sec:benchmarks}. The comparison itself is detailed in
Sections~\ref{sec:rwd}--\ref{sec:syn}. We first
discuss the evaluation
methodology in Section~\ref{sec:methodology}.



\subsection{Methodology}
\label{sec:methodology}
\input{sections/methodology.tex}


\subsection{Benchmarks}
\label{sec:benchmarks}
\input{sections/benchmarks.tex}

\subsection{\rwd experiments}
\label{sec:rwd}
\input{sections/rwd-experiments.tex}


\subsection{\nrwd experiments}
\label{sec:rwd:noise}
\input{sections/nrwd-experiments.tex}


\subsection{\syn experiments}
\label{sec:syn}
\input{sections/syn-experiments.tex}





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main/main"
%%% End:

